User Inference Attacks on Large Language Models

Fine-tuning is a common and effective method for tailoring large language models (LLMs) to specialized tasks and applications. In this paper, we study the privacy implications of fine-tuning LLMs on user data. To this end, we consider a realistic threat model, called user inference, wherein an attacker infers whether or not a user's data was used for fine-tuning. We design attacks for performing user inference that require only black-box access to the fine-tuned LLM and a few samples from a user which need not be from the fine-tuning dataset. We find that LLMs are susceptible to user inference across a variety of fine-tuning datasets, at times with near perfect attack success rates. Further, we theoretically and empirically investigate the properties that make users vulnerable to user inference, finding that outlier users, users with identifiable shared features between examples, and users that contribute a large fraction of the fine-tuning data are most susceptible to attack. Based on these findings, we identify several methods for mitigating user inference including training with example-level differential privacy, removing within-user duplicate examples, and reducing a user's contribution to the training data. While these techniques provide partial mitigation of user inference, we highlight the need to develop methods to fully protect fine-tuned LLMs against this privacy risk.

==> figures/attacker_knowledge.tex <==
\begin{figure}[bth!]
\centering
% \includegraphics[width=\linewidth]{images/figures_attacker_knowledge.pdf}
\includegraphics[width=\linewidth]{images_v2/attacker_knowledge.pdf}
\caption{\small
\textbf{Attack performance vs. attacker knowledge}: As we increase the number of examples given to the attacker, the attack performance increases across all three datasets. 
% At each level of attacker knowledge, we shade the AUROC standard deviation over $100$ random draws of attacker examples.
The shaded area denotes the std over $100$ random draws of attacker examples.
} \label{fig:attacker_knowledge}
\end{figure}

==> figures/canary_gradient_norms.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/figures_canary_gradient_norms.pdf}
\caption{\nikhil{Better to keep this as a separate figure or add it as a subplot into the gradient clipping mitigation plot?}}
\end{figure}

==> figures/canary_lengths.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/figures_canary_lengths.pdf}
\caption{}
\end{figure}

==> figures/canary_num_docs.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/figures_canary_num_docs.pdf}
\caption{}
\end{figure}

==> figures/dataset_hists.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/figures_dataset_hists.pdf}
\caption{\small
\textbf{Per-user statistics}: Histograms of the number of documents per user for each dataset.
}
\label{fig:dataset_hists}
\end{figure}

==> figures/gradient_clipping.tex <==
\begin{figure}
\centering
% \includegraphics[width=\linewidth]{images/figures_gradient_clipping.pdf}
\includegraphics[width=\linewidth]{images_v2/figures_gradient_clipping2.pdf}
\caption{\small
Mitigation with gradient clipping. \textbf{Left}: Attack effectiveness for canaries with different shared substring lengths with gradient clipping ($125$M model, CC News). \textbf{Right}: The distribution of gradient norms for canary examples and real examples.
\vspace{-2em}
} \label{fig:gradient_clipping}
\end{figure}

==> figures/reddit_data_size.tex <==
\begin{figure}[bth!]
\centering
% \includegraphics[width=\linewidth]{images/figures_attacker_knowledge.pdf}
\includegraphics[width=\linewidth]{images_v2/reddit_data_fraction_comparison.pdf}
\caption{\small
\textbf{Effect of increasing the fraction of data contributed by each user}: 
} \label{fig:reddit_data_size}
\end{figure}

==> sections/OLD/attack.tex <==
\section{User Inference Attacks: Old}

Background on LLM, fine-tuning with user data

\subsection{Threat Model}
\nikhil{Need to make the notation consistent between this subsection and Attack Strategy.}
Modern LLMs are trained and fine-tuned on user-provided data (e.g., posts, emails, messages, etc.)~\cite{xu2023federated}. Fine-tuned models  achieve higher performance on tasks such as smart compose or text generation compared to general-purpose LLMs~\cite{liu2022fewshot}. For example, a company might fine-tune an LLM on a corpus of email data to provide a service of email smart compose to its users~\cite{}. Membership inference (MI) attacks have been designed for LLMs~\cite{}, but they assume the attacker has full knowledge of a text sample $x$  to determine whether $x$ was part of the model’s training data. For LLMs, it might be challenging for attackers to get access to exact samples of training text. We introduce instead a new, more realistic privacy threat model for LLMs, called User Inference (UI), which relaxes the assumptions on the adversary knowledge. 

In our setting, the attacker is given access to a fine-tuned  model $\theta$ and a set of documents $D_A$ from a particular \emph{target user} $U$. The attacker can query the fine-tuned LLM in a \emph{black-box} manner and obtain the model's likelihood on a sequence of tokens $P_{\theta}(x)$. Importantly, the attacker does not know the model architecture or the model parameters, which are typically proprietary to companies training LLMs.  The attacker’s goal is to determine whether the target user $U$ participated into the model's training set. 
Crucially, while the target user may have contributed some of their data to the training dataset (denoted $D_U$), the samples $D_A$ that the attacker has access to were not part of the training data. In general, we assume that $D_U$ and $D_A$ are disjoint, but come from the same distribution. In our example email scenario, it is perfectly reasonable to assume that an attacker has received a few emails from the target user, but the attacker does not have exact knowledge of the emails included in the fine-tuning set of the model.

%Attackers might generate user-specific prompts to extract sensitive information from target users, or try to poison the victim user's dataset.

%- Black-box: compute loss on token (does any existing LLM provide this API?)

%How to generalize attack if access only to generative API? 

\subsection{Attack Strategy}
To perform an inference attack, either at the example level (Membership Inference) or the user level (User Inference), an attacker defines an attack statistic that they compute for each example/user, with the goal of distinguishing examples/users that were part of the training set (held-in) from ones that were not (held-out) \citep{shokri2017membership}.

A commonly used attack statistic for membership inference is the likelihood of a sample under the target model, $\theta$, normalized by the likelihood of a reference model, $\theta_{\text{ref}}$, that has not trained on that sample \citep{Carlini_Memorization, mireshghallah-etal-2022-quantifying, watson2022importance}. \nikhil{Do we need to explain the intuition behind difficulty calibration here? This is a pretty well-understood method that's used in a bunch of different papers.}
\begin{align} \label{eq:mi}
    s_{\text{MI}}(x) = \log  \frac{P(x \mid \theta)}{P(x \mid \theta_{\text{ref}})} 
\end{align}

In this work, we adapt this Membership Inference attack statistic to score \emph{users} rather than single examples. Specifically, we define a User Inference attack statistic as the expected Membership Inference statistic over documents drawn from a particular user's data distribution.

\begin{align} \label{eq:dist_ui}
    s_{\text{UI}}(P_U) = \mathbb{E}_{x \sim P_U} \bigl[ s_{\text{MI}}(x) \bigr]
\end{align}

In practice, an attacker estimates this user-level attack statistic with a sample mean over a set of examples, $D_U$, drawn from that user's data distribution.

\begin{align} 
\label{eq:sample_ui}
    \hat{s}_{\text{UI}}(D_U) = \frac{1}{\lvert D_U \rvert} \sum_{x \in D_U} s_\text{MI}(x) 
\end{align}

%- Likelihood of each document (computed as sum of likelihood of tokens in document) normalized by reference model

\begin{comment}
Motivate design decisions:
\begin{enumerate}

\item Why use normalization / calibration for computing document score 

Compare against a baseline using average loss over all documents / not include the normalization to motivate difficulty calibration

\item Describe aggregation function for a set of documents from the same user: mean / max / min
\end{enumerate}
\end{comment}

\begin{comment}
\subsection{Mitigations}

Discuss several mitigation strategies: mini-bath clipping, outlier removal, bounding user contribution 
\end{comment}

==> sections/OLD/introduction.tex <==
\section{Introduction}

%LLMs: pre-training and fine-tuning
Modern large language models (LLMs) such as GPT-4~\citep{openai2023gpt4}, PaLM2~\citep{anil2023palm}, and LLaMA~\cite{touvron2023llama} are large-scale general-purpose models  trained on terabytes of crowdsourced text from the Internet. These models, sometimes called \emph{foundation models}, learn to generate high-quality text given a user-provided prompt. It has become common to fine-tune these models  on  downstream tasks, such as machine translation, question answering, conversational agents, on which they  achieved  remarkable results~\cite{}. 
%Privacy attacks in LLM: MI / Memorization

Given the trend of scaling  LLMs in terms of their parameters and training set size, it becomes crucial to study privacy attacks in LLMs to understand if these models leak sensitive information about their training datasets. Early work on LLM privacy identified the risk of \emph{training data memorization}, demonstrating that larger models have a tendency to memorize their training sets~\cite{Carlini_Memorization,NEURIPS2022_fa0509f4}. Existing privacy attacks on LLMs can be grouped into two categories: \emph{membership inference} (MI), in which the attacker obtains access to a data sample (usually a sequence of tokens) and would like to determine if it was part of training~\cite{mireshghallah-etal-2022-quantifying,mattern-etal-2023-membership,code_leakage}; and \emph{extraction attacks} in which the adversary's goal is to reconstruct the training data by prompting the model with different prefixes~\cite{Carlini_Memorization,pii_leakage}. Most of these attacks assume a \emph{black-box} API access to the LLM model in which attackers can compute loss on samples of their choice, without knowledge of the model architecture or parameters. These attacks do not take into consideration the users who contributed the data samples to the training set, but in reality many fine-tuning LLM tasks leverage user-provided datasets such as emails or documents. 

%Membership inference attacks are not realistic in the context of LLMs as it is difficult to get access to exact training sample 

%Introduce new user inference attack on LLMs
In this paper, we identify a new relevant and realistic privacy attack vector for LLMs fine-tuned on user data. In our \emph{user inference} (UI) attack model, the attacker's goal is to determine if a particular target user participated in fine-tuning the LLM by getting black-box access to the fine-tuned model. UI lifts the concept of MI from individual text samples to users contributing their datasets to training or fine-tuning LLMs. Importantly, there is a fundamental difference between UI and MI: MI requires access to \emph{exact} training samples, while UI relies only on knowledge of a small set of samples of the target user that were not necessarily part of the training set. Therefore, UI results in a more realistic threat model than MI, as it is more reasonable for attackers to get access to a few documents from a target user (such as emails or posts) than assuming knowledge of training samples. User inference reveals a new type of privacy violation in LLMs that exposes user participation in the language model's fine-tuning sets. By itself, this could be a relevant privacy threat if the fine-tuning task reveals sensitive information about participating users (for instance, model is fine-tuned on users with a rare disease). Additionally, user inference might enable even more damaging attacks such as sensitive data extraction or poisoning, similarly to how membership inference has been used as a building block  for  extracting  training data from LLMs~\cite{Carlini_Memorization}. 

The technical contributions of the paper are: (1) We introduce a new black-box user inference privacy threat model for LLMs, in which adversaries aim to  infer user participation in training under realistic assumptions; (2) We design user inference attacks that compute user-level scores by combining normalized likelihoods on a set of documents and show that difficulty calibration is important for improving the attack success; (3) We evaluate the attack on three datasets using public GPT-Neo models and perform analysis of attack performance for several user populations, including randomly selected users, out-of-distribution users, and synthetically-generated canary users; (4) We evaluate several efficient mitigation strategies to understand how the attack might be thwarted.

\begin{comment}
\begin{itemize}
    \item Introduction of new user-level privacy threat model for LLMs: Infer user participation in training with less knowledge
    \item Attack strategy inspired from MI, but adapted to user inference. Show that difficulty calibration is important
    \item Evaluation of attack on three datasets using public GPT-Neo models. Perform analysis of attack success for several user populations, including randomly selected users, users that are part of the tail distribution, and synthetically-generated, canary users. 
    \item Evaluate several efficient mitigation strategies to understand how the attack might be thwarted. 
\end{itemize}
\end{comment}





==> sections/related_v2.tex <==
\section{Related Work}

%- Related Work on MI/Memorization with focus on LLMs

Over the years, a range of ML privacy attacks  with different objectives have been studied~\cite{NIST_report}: \emph{membership inference} attacks determine if a particular data sample was part of a model's training set~\cite{shokri2017membership,yeom_mi,LiRA,enhanced_mi,watson2022importance,choquette2021label,jagielski2023students}; \emph{data reconstruction} aims to exactly reconstruct the training data of a model (typically for a discriminative model)~\cite{haim2022reconstructing}; and \emph{extraction} attacks  aim to extract training data from generative models like LLMs~\cite{Carlini_Memorization,pii_leakage,ippolito2022preventing,anil2023palm,kudugunta2023madlad}.

Most membership inference attacks have studied classifiers~\cite{shokri2017membership,yeom_mi,LiRA,choquette2021label,jagielski2023students}, but recently membership inference attacks on LLMs have been proposed~\cite{mireshghallah-etal-2022-quantifying,mattern-etal-2023-membership,debenedetti2023privacy}. \citet{mireshghallah-etal-2022-quantifying} introduce a likelihood ratio-based attack on LLMs, designed for masked language models, such as BERT. \citet{mattern-etal-2023-membership} propose an attack that compares the likelihood of a sample against the average likelihood of a set of neighboring samples, thus relaxing the assumption that the attacker knows the training distribution, which is commonly used in membership inference.
\citet{debenedetti2023privacy} study how systems built on LLMs may amplify membership inference.

Recently a number of extraction attacks have been studied that use membership inference as a subroutine \cite{Carlini_Memorization,kandpal2022deduplicating,pii_leakage}. \citet{Carlini_Memorization} use a perplexity-based membership inference attack to extract training data from GPT-2. Their attack prompts the LLM to generate sequences of text, and then uses membership inference to identify sequences copied from the training set. \citet{kandpal2022deduplicating} study the same attack and find that the sequences extracted from LLMs tend to be repeated often in the training data. \citet{pii_leakage} develop techniques to specifically extract personal identifiable information (PII) from fine-tuned versions of GPT-2 and estimate the amount of PII leakage in these models.

After~\citet{Carlini_Memorization} discovered GPT-2 can be prompted to regurgitate thousands of samples from its training data, the phenomenon of memorization in LLMs has been  studied extensively~\cite{zhang2021counterfactual,NEURIPS2022_fa0509f4,biderman2023emergent,lee2021deduplicating,anil2023palm}. Past work has found that memorization scales with model size~\cite{carlini2023quantifying}, memorized samples may eventually be forgotten~\cite{jagielski2022measuring}, and memorization can exist even on models trained for specific restricted use-cases like translation~\cite{kudugunta2023madlad}.

While most work studying privacy of LMs has focused on privacy at the level of individual samples or sequences, our work, along with \citet{inan2021training} and \citet{song2019auditing} study user-level privacy when LMs are trained on user-stratified datasets. \citet{song2019auditing} study a user-level generalization of membership inference, where an attacker gains access to a set of samples from a user and must determine whether those samples were part of the training data. \citet{inan2021training} introduce several metrics to measure if a user's confidential data is leaked by an LLM by counting the number of sequences generated by the model that uniquely appear in the user's training set.

Compared to previously studied threat models, the user inference threat model introduced in this paper assumes a weaker adversary and measures a new type of privacy leakage. Like \citet{song2019auditing}, user inference focuses on exposing whether a certain user's data was used for fine-tuning. However, compared to both sample and user-level membership inference, user inference relaxes the assumption that the attacker has access to exact training samples. Instead user inference only assumes that the attacker has access to \emph{some data} from a user, not necessarily data that was used for training. Compared to extraction attacks, user inference does not require memorization of exact training samples to work. Instead, user inference requires that a model learns generalizable patterns from a user's data that are unique to that user's data distribution. These properties make user inference a novel and realistic attack vector in the space of LLM privacy attacks. 

% Another difference between user inference and existing privacy attacks is the granularity of inference. The above attacks in LLMs perform inference on text sequences, not necessarily associated to a particular user, while user inference attacks infer user participation in training. The only user-level privacy attacks against LMs we are aware of are \citet{inan2021training} and \citet{song2019auditing}. \citet{inan2021training} introduce several metrics to measure if a user's confidential data is leaked by the LLM by counting the number of sequences generated by the model that uniquely appear in the user's training set. The goal of our user inference attack is orthogonal: it is to identify which users participated in LLM training or fine-tuning. Once a user is identified by user inference, methods from \citet{inan2021training} can be used to estimate the amount of  privacy leakage. \citet{song2019auditing} study methods for inferring whether a user's data was part of the training set, but they assume that the attacker has access to exact samples in the training set. User inference relaxes this assumption by assuming the attacker has data from a user without requiring that the samples were part of training.



==> sections/results.tex <==
\subsection{User Inference: Results and Properties} \label{sec:results}

We examine how user inference is impacted by factors such as the amount of user data and attacker knowledge, the model scale, as well as the connection to overfitting.


% In the remainder of this paper we empirically study user inference attacks using the attack statistic from Section~\ref{sec:attack}.

\myparagraph{Attack Performance}
We attack GPT-Neo $125$M fine-tuned on each of the three fine-tuning datasets and evaluate the attack performance. 
We see from \Cref{fig:hists_aurocs} that the user inference attacks on all three datasets achieve non-trivial performance, with the attack AUROC varying between $88\%$ (Enron) to $66\%$ (CC News) and $56\%$ (Reddit).


\input{figures/training_aurocs}
\input{figures/model_scaling}
\input{figures/attacker_knowledge}

The disparity in performance between the three datasets can be explained in part by the intuition from \Cref{thm:analysis}, which points out two factors.
First, a larger fraction of data contributed by a user makes user inference easier. The Enron dataset has fewer users, each of whom contributes a significant fraction of the fine-tuning data (cf.~\Cref{tab:datasets}), 
% This makes user inference easier.
while, the Reddit dataset has a large number of users, each with few datapoints.
Second, distinct user data makes user inference easier. Emails are more distinct due to identifying information such as names (in salutations and signatures) and addresses, while news articles or social media comments from a particular user may share more subtle features like topic or writing style.

\myparagraph{The Effect of the Attacker Knowledge}
We examine the effect of the attacker knowledge
(the amount of user data used by the attacker to compute the test statistic) in \Cref{fig:attacker_knowledge}. First, we find that  more attacker knowledge leads to higher attack AUROC and lower variance in the attack success. For CC News, the AUROC increases from $62.0 \pm 3.3 \%$ when the attacker has only one document to $68.1\pm 0.6\%$ at 50 documents. The user inference attack already leads to non-trivial results with an attacker knowledge of \emph{one document per user} for CC News (AUROC $62.0\%$) and Enron Emails (AUROC $73.2\%$).
Overall, the results show that an attacker does not need much data to mount a strong attack, and more data only helps.


\myparagraph{User Inference and User-level Overfitting}
It is well-established that overfitting to the training data is sufficient for successful membership inference~\cite{yeom_mi}. We find that a similar phenomenon holds for user inference, which is enabled by \emph{user-level overfitting}, i.e., the model overfits not to the training samples themselves, but rather the \emph{distributions} of the training users.

We see from \Cref{fig:training_run} that the validation loss of held-in users continues to decrease for \emph{all 3 datasets}, while the loss of held-out users increases. These curves display a textbook example of overfitting, not to the training data (since both curves are computed using validation data), but to the distributions of the training users. Note that the attack AUROC improves with the widening generalization gap between these two curves.
Indeed, the Spearman correlation between the generalization gap and the attack AUROC is at least $99.4\%$ for all datasets.
This demonstrates the close relation between user-level overfitting and user inference.

\input{figures/canary_attacks}

\myparagraph{Attack Performance and Model Scale}
Next, we investigate the role of model scale in user inference using the GPT-Neo $125$M and $1.3$B on the CC News dataset. 

\Cref{fig:model_scale} shows  that the attack AUROC is nearly identical for the $1.3$B model ($65.3\%$) and $125$M model ($65.8\%$). While the larger model achieves better validation loss on both held-in users ($2.24$ vs. $2.64$) and held-out users ($2.81$ vs. $3.20$), the generalization gap is nearly the same for both models ($0.57$ vs. $0.53$). This shows a qualitative difference between user and membership inference, where attack performance reliably increases with model size in the latter \cite{carlini2023quantifying,NEURIPS2022_fa0509f4,kandpal2022deduplicating,mireshghallah-etal-2022-quantifying,anil2023palm}.

\input{figures/gradient_clipping}


\subsection{User Inference in the Worst-Case} \label{sec:canaries}

The disproportionately large downside to privacy leakage necessitates looking beyond the average-case privacy risk to worst-case settings.
Thus, we analyze attack performance on datasets containing synthetically generated users, known as \emph{canaries}.
There is usually a trade-off between making the canary users realistic and worsening their privacy risk. We intentionally err on the side of making them realistic to illustrate the potential risks of user inference.


To construct a canary user, we first sample a real user from the dataset and insert a particular substring into each of that user's examples. The substring shared between all of the user's examples is a contiguous substring randomly sampled from one of their documents (for more details, see \Cref{appendix:experiments}). We construct $180$ canary users with shared substrings ranging from $1$-$100$ tokens in length and inject these users into the Reddit and CC News datasets. 
We do not experiment with synthetic canaries in Enron Emails, as the attack AUROC already exceeds $88\%$ for real users. 

\Cref{fig:canaries} (left) shows that the attack is more effective on canaries than real users, and increases with the length of the shared substring. 
A short shared substring is enough to significantly increase the attack AUROC from $63\%$ to $69\%$ (5 tokens) for CC News and $56\%$ to $65\%$ for Reddit (10 tokens).

These results raise a question if canary gradients can be filtered out easily (e.g., using the $\ell_2$ norm). However, \Cref{fig:gradient_clipping} (right) shows that the gradient norm distribution of the canary gradients and those of real users are nearly indistinguishable.
This shows that our canaries are close to real users from the model's perspective, and thus hard to filter out. This experiment also demonstrates the increased privacy risk for users who use, for instance, a short and unique signature in emails or characteristic phrases in documents.
% Regarding the canary identifiablity, we plot the distribution of gradient norms for canary and real examples in the right plot of Figure~\ref{fig:gradient_clipping}, which demonstrates that canary examples are similar to real-user examples. This shows that our canaries are close to real users and much more realistic than canaries with randomly generated text, which would be very identifiable and can be easily sanitized in the fine-tuning phase. This finding demonstrates that the privacy risk of users participating in LLM fine-tuning can be increased significantly for particular users (those who use, for instance,  a short, unique signature in emails or documents   consistently). Analyzing the susceptibility of LLM fine-tuning to other classes of synthetically generated users is an interesting topic for future work. 


\subsection{Mitigation Strategies} \label{sec:defenses}
Finally, we investigate existing techniques for limiting the influence of individual examples or users on model fine-tuning as methods for mitigating user inference attacks.

\myparagraph{Gradient Clipping}
Since we consider fine-tuning that is oblivious to the user-stratification of the data, one can limit the model's sensitivity by clipping the gradients per batch \cite{pascanu2013difficulty} or per example \cite{Abadi_2016}. \Cref{fig:gradient_clipping} (left) plots its effect for the $125$M model on CC News: neither batch nor per-example gradient clipping have any effect on user inference. \Cref{fig:gradient_clipping} (right) tells us why: canary examples do not have large outlying gradients and clipping affects real and canary data similarly. Thus, gradient clipping is an ineffective mitigation strategy.

\myparagraph{Early Stopping}
The connection between user inference and user-level overfitting from \Cref{sec:results} suggests that early stopping, a common heuristic used to prevent overfitting~\cite{caruana2000overfitting}, could potentially mitigate user inference. Unfortunately, we find that $95\%$ of the final AUROC is obtained quite early in training: $15$K steps ($5\%$ of the fine-tuning) for CC News and $90$K steps ($18\%$ of the fine-tuning) for Reddit, see \Cref{fig:training_run}.
% $90$K steps ($27\%$ of the fine-tuning) for ArXiv. 
Typically, the overall validation loss still decreases far after this point. This suggests an explicit tradeoff between model utility (e.g., in validation loss) and privacy risks from user inference.

\myparagraph{Data Limits Per User}
Since we cannot change the fine-tuning procedure, we consider limiting the amount of fine-tuning data per user.
\Cref{fig:canaries} (right two) show that this can be effective. For CC News, the AUROC for canary users reduces from $77\%$ at $100$ fine-tuning documents per user to almost random chance at $5$ documents per user.
A similar trend also holds for Reddit.

\myparagraph{Data Deduplication}
Since data deduplication can mitigate membership inference~\cite{lee2021deduplicating,kandpal2022deduplicating}, we evaluate it for user inference. CC News is the only dataset in our suite with within-user duplicates (Reddit and Enron are deduplicated in the preprocessing; see \Cref{sec:a:expt:ds}), so we use it for this experiment.\footnote{
    Although each article of CC News from HuggingFace Datasets has a unique URL, the text of $11\%$ of the articles has exact duplicates from the same domain.
    See \S\ref{sec:ccnews-dup} for examples.
}
The deduplication reduces the attack AUROC from $65.7\%$ to $59.1\%$. The attack ROC curve of the deduplicated version is also uniformly lower, even at extremely small FPRs (\Cref{fig:dedup}). 

Thus, data \emph{repetition} (e.g., due to poor preprocessing) can exacerbate user inference. However, the results on Reddit and Enron Emails (no duplicates) suggest that deduplication alone is insufficient to fully mitigate user inference.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{images_v2/figure_dedup.pdf}
    \caption{\small Effect of data deduplication per-user on CC News. \Cref{tab:ccnews-dedup} in \Cref{appendix:expt-results} gives TPR values at low FPR.}
    \label{fig:dedup}
\end{figure}

\myparagraph{Example-level Differential Privacy (DP)}
DP~\cite{DMNS} gives provable bounds on privacy leakage. We study how example-level DP, which protects the privacy of individual \emph{examples}, impacts \emph{user} inference. We train the 125M model on Enron Emails using DP-Adam, a variant of Adam that clips per-example gradients and adds noise calibrated to the privacy budget $\varepsilon$. We find next that example-level DP can somewhat mitigate user inference while incurring increased compute cost and a degraded model utility.


Obtaining good utility with DP requires large batches and more epochs~\citep{ponomareva2023dp}, so we use a batch size of $1024$, tune the learning rate, and train the model for $50$ epochs ($1.2K$ updates), so that each job runs in $24$h (in comparison, non-private training takes $1.5$h for $7$ epochs). Further details of the tuning are given in \Cref{appendix:dp-tuning}.

\Cref{tab:enron_dp} shows a severe degradation in the validation loss under DP. For instance, a loss of $2.67$ at the weak guarantee of  $\varepsilon=32$ is  surpassed after just $1/3$\textsuperscript{rd} of an epoch of non-private training; this loss continues to reduce to $2.43$ after $3$ epochs.
In terms of attack effectiveness, example-level DP reduces the attack AUROC and the TPR at FPR $=5\%$, while the TPR at FPR $=1\%$ remains the same or gets worse.
Indeed, while example-level DP protects individual examples, it can fail to protect the privacy of \emph{users}, especially when they contribute many examples.
This highlights the need for scalable algorithms and software for fine-tuning LLMs with \emph{DP at the user-level}. Currently,  user-level DP algorithms have been designed for small models in federated learning, but do not yet scale to LLMs.

\input{tables/example_level_dp}

\myparagraph{Summary}
Our results show that user inference is hard to mitigate with common heuristics.
Careful deduplication is necessary to ensure that data repetition does not exacerbate user inference.
Enforcing data limits per user can be effective but this only works for data-rich applications with a large number of users. Example-level DP can offer moderate mitigation but at the cost of increased data/compute and degraded model utility.
Developing an effective mitigation strategy that also works efficiently in data-scarce applications remains an open problem.
% This is promising and it highlights the need to develop more rigorous mitigations for user inference attacks, including user-level differential privacy, which is currently a challenging open problem for LLMs. 










